On Efficient Constructions of Checkpoints

Efficient construction of checkpoints/snapshots is a critical tool for training and diagnosing deep learning models. In this paper, we propose a lossy compression scheme for checkpoint constructions (called LC-Checkpoint). LC-Checkpoint simultaneously maximizes the compression rate and optimizes the recovery speed, under the assumption that SGD is used to train the model. LC-Checkpointuses quantization and priority promotion to store the most crucial information for SGD to recover, and then uses a Huffman coding to leverage the non-uniform distribution of the gradient scales. Our extensive experiments show that LC-Checkpoint achieves a compression rate up to $28\times$ and recovery speedup up to $5.77\times$ over a state-of-the-art algorithm (SCAR).

==> model.tex <==

\newpage
\onecolumn
\section{Theoretical model}

{\color{blue} Be careful of notation consistency.} 

\myparab{The dynamic of the process.} We assume that $x^* = 0$. The series $\{x_t\}_{t \geq 1}$ can be described by a generative process
\begin{equation}
    x_{t + 1} = \eta x_t + z_t, 
\end{equation}
where $\eta < 1$ and $z_t$ models the noise produced from the stochastic gradient descent algorithm. We also assume that $\|z_t\|_t$ is bounded by $\|x_t\|_2$ (i.e., the noise term decays as $x_t$ converges to $0$). 

Now we assume that we perform a delta-encoding compression algorithm, where 
\begin{align*}
    \delta_{t + 1} & = x_{t + 1} - x_t  \\
    & = \eta x_t + z_t - x_t = (\eta - 1)x_t + z_t. 
\end{align*}

The information lost can be described as a function of $f(\delta)$. In other words, we examine the following dynamics
\begin{equation}
    x_{t + 1} = \eta x_t + z_t + f(\delta_t). 
\end{equation}
Our goal is to examine how $f(\delta_t)$ will imacge the convergence behavior. 

\myparab{Exercise 1.} We first aim to understand the convergence behavior of the original algorithm. 
\begin{equation}
    x_{t + 1} = \eta x_t + z_t.
\end{equation}
We consider two specific settings: 

\mypara{Setting 1a.} We assume that $x_t$ is 1-dimensional. Can we show the convergence rate. 

\mypara{Setting 1b.} We assume that $x_t$ is high dimensional. Can we show the convergence rate? 

We have the following observation: if $\|x_t\| \leq \|x'_t\|$, then there is a way to couple $\{x_t\}_t$ and $\{x'_t\}_t$ such that $\|x_{\tau}\| \leq \|x'_{\tau}\|$ for all $\tau \geq t$. {\color{blue} Question: does this hold only for the 1-dimensional setting, or also hold for high dimensional settings?}

\myparab{Exercise 2.} $f(\delta)$ is to keep all the top $k$ items. 

\myparab{Exercise 3.} $f(\delta)$ is a randomized  rounding. 

\myparab{Exercise 4.} $f(\delta)$ is zero mean with bounded variance.

\myparab{Compression of $f(\delta)$.} Compression of $f(\delta)$ requires us to co-optimize a loss function and the entropy. We assume two kinds of operations. \emph{(i)} Quantization, and \emph{(ii)} Huffman coding. 

We have these loss functions: 
\begin{enumerate}
    \item Loss function is MSE. 
    \item Loss function is minimizing ratio sum (take ratio between the compressed number and the original number; then sum up the ratios). 
    \item Loss function is minimizing maximum ratio.  
\end{enumerate}

\myparab{Example. Minimizing the $\ell_2$-loss.} Let $I_1, I_2, \dots, I_k$ be a partition of intervals of the support of $x_i$. Let $S_1, \dots, S_k$ be that $S_i = \{\delta_j: \delta_j \in I_i\}$. Let $s_i = \frac{1}{|S_i|} \sum_{j \in S_i}\delta_j$ (this is the mean of the points in $S_i$). Let $p_i = |S_i|/n$ (recall that $n$ is the number of points or dimension of $\delta_j$). The MSE cost is 
\begin{equation}
    E = \sum_{i \leq k}\sum_{\delta_j \in S_i}\|(\delta_j - s_i)\|^2. 
\end{equation}

The entropy is $\lambda H = \sum_{i \leq p}p_i \log(1/p_i)$. Let the cost function be $E + \lambda H$. $\lambda$ is a tunable parameter. 

\mypara{Observation 1.} We can run a dynamic programming to solve the problem. 

\mypara{Observation 2.} If there are too many elements, we can do a saimplying (or sampling plus top-$k$). 




==> toremove.tex <==

\cite{han2015deep}
\begin{itemize}
    \item Taking snapshot is an important task. 
    \item Application 1. Recovery from crashes. (Training usually takes long time (and easy to crash) that requires fault tolerance support.)
    \item Application 2. diagnosis deep learning models; 
    \item Why it is challenging. 
    \item Summary of our contribution. 
\end{itemize}

\iffalse
Machine learning (ML) application is typically stateful and long-running. Interruption happens often in this kind of job due to hardware failure, software bugs, etc. It's essential to make the checkpoint periodically because rebuilding the state from scratch is time-consuming. Also, ML application behaves variedly among different executions thus making a recovery from a specific checkpoint is important for debugging. The checkpoint mechanism for ML application has been well studied by previous works. These approaches provide strong consistency semantics. They snapshot the full picture of the application state which dramatically inflates the checkpoint's size, resulting in massive extra overhead. For example, the checkpoint size of AlexNet in MXNET is 178MB and the one of VGG-19 is 229MB.

However, ML application doesn't require such a strong consistency model because of its self-correcting characteristics. ML algorithms often are iterative. For each iteration, the ML application does the calculation based on the current state and obtains a set of parameter values that is closer to the convergent target. It repeats the step until achieving a set of optimal values which has reached the convergent state. The small calculation errors happened during the runtime are eliminated by successive optimizing procedure and perform as more iterations of execution.
\fi

Compression of model states is a new technical problem that requires addressing cross-cutting constraints from information theory, learning algorithm, and system design. We need to simultaneously leverage statistical patterns encoded in the model state and factor in how the model states interact with a learning algorithm (more specifically, stochastic gradient type algorithm in the deep learning setting). This means neither standard lossy compression algorithms nor recently developed model compression algorithms directly work in our setting. Standard lossy compression algorithms aim to minimize reconstruction error but our end goal is to enable a learning algorithm to ``quickly recover. '' Model compression techniques aim to transform a (static) model into a simpler one while ensuring the forecasts are not perturbed much whereas in our setting we need a reliable coding scheme that functions well throughout the entire dynamic process of learning, an orthogonal and perhaps more challenging goal. In addition, our algorithms need to be efficient and scalable because taking snapshots can be a frequent operation. 

